What does it mean to be language-agnostic? Probing multilingual sentence encoders for typological properties

Multilingual sentence encoders have seen much success in cross-lingual model transfer for downstream NLP tasks. Yet, we know relatively little about the properties of individual languages or the general patterns of linguistic variation that they encode. We propose methods for probing sentence representations from state-of-the-art multilingual encoders (LASER, M-BERT, XLM and XLM-R) with respect to a range of typological properties pertaining to lexical, morphological and syntactic structure. In addition, we investigate how this information is distributed across all layers of the models. Our results show interesting differences in encoding linguistic variation associated with different pretraining strategies.

==> emnlp2020-templates/table_variation.tex <==
\setlength{\tabcolsep}{2.6pt}

\begin{table}[t!]
\small
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\midrule
&\multicolumn{7}{c|}{Train}&\multicolumn{7}{c}{Test}\\
\hline
\T & ru & da &cs & pt & hi  & mk& it& uk& sv & pl & es & mr & bg & fr \\
\midrule
37A & \cellcolor{fandango!75}&  \cellcolor{yellowish}&\cellcolor{fandango!75} & \cellcolor{teal}&\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{teal} & \cellcolor{fandango!75}&\cellcolor{yellowish} &\cellcolor{fandango!75} & \cellcolor{teal}&\cellcolor{fandango!75} & \cellcolor{teal}&\cellcolor{teal}     \\
38A  &\cellcolor{fandango!75}&  \cellcolor{yellowish} &\cellcolor{fandango!75} & \cellcolor{teal}& \cellcolor{fandango!75}&\cellcolor{White!50} &\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{fandango!75} & \cellcolor{White!50}& \cellcolor{teal}    \\
51A &\cellcolor{teal} &\cellcolor{teal}  & \cellcolor{teal}&\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{White!50} & \cellcolor{White!50}&\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{White!50} & \cellcolor{White!50}    \\
70A &\cellcolor{teal} & \cellcolor{fandango!75} & \cellcolor{teal} &\cellcolor{yellowish} & \cellcolor{teal} &\cellcolor{teal}  &\cellcolor{yellowish} &\cellcolor{teal}  &\cellcolor{fandango!75} &\cellcolor{teal}  &\cellcolor{teal}  &\cellcolor{fandango!75} &\cellcolor{teal}  & \cellcolor{yellowish}    \\
71A & \cellcolor{teal}&\cellcolor{teal}  &\cellcolor{teal} &\cellcolor{fandango!75} & \cellcolor{greenish}& \cellcolor{yellowish}&\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{yellowish} &\cellcolor{yellowish} & \cellcolor{teal}    \\
72A & \cellcolor{teal}&\cellcolor{teal}  &\cellcolor{teal} &\cellcolor{teal} & \cellcolor{teal}& \cellcolor{fandango!75}&\cellcolor{teal} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{fandango!75} & \cellcolor{teal}   \\
79A & \cellcolor{teal}&\cellcolor{White!50} &\cellcolor{teal} &\cellcolor{White!50} &\cellcolor{White!50}&\cellcolor{fandango!75} &\cellcolor{White!50} & \cellcolor{teal} &\cellcolor{White!50} &  \cellcolor{teal} &\cellcolor{White!50}&\cellcolor{White!50} & \cellcolor{fandango!75} &\cellcolor{White!50}     \\
79B  &\cellcolor{fandango!75}&\cellcolor{White!50} &\cellcolor{teal} &\cellcolor{White!50} &\cellcolor{White!50}&\cellcolor{yellowish} &\cellcolor{White!50} & \cellcolor{teal} &\cellcolor{White!50} &  \cellcolor{teal} &\cellcolor{White!50}&\cellcolor{White!50} & \cellcolor{yellowish} &\cellcolor{White!50}     \\
82A &  \cellcolor{teal}&\cellcolor{teal}  &\cellcolor{teal} &\cellcolor{teal} & \cellcolor{teal}& \cellcolor{teal}&\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{fandango!75} & \cellcolor{teal}   \\
86A &  \cellcolor{White!50}&\cellcolor{fandango!75}  &\cellcolor{yellowish} &\cellcolor{teal} & \cellcolor{fandango!75}& \cellcolor{yellowish}&\cellcolor{teal} &\cellcolor{White!50} &\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{yellowish} & \cellcolor{teal}   \\
92A &\cellcolor{yellowish} &\cellcolor{teal}  &\cellcolor{teal} & \cellcolor{fandango!75}& \cellcolor{White!50}& \cellcolor{White!50}&\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{teal} & \cellcolor{White!50}&\cellcolor{White!50} &\cellcolor{fandango!75}     \\
93A & \cellcolor{teal}& \cellcolor{teal} &\cellcolor{fandango!75} &\cellcolor{White!50}  &\cellcolor{fandango!75} &\cellcolor{White!50}  &\cellcolor{White!50}  &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{White!50}  &\cellcolor{fandango!75} &\cellcolor{White!50}  &\cellcolor{White!50}      \\
116A &\cellcolor{teal} &\cellcolor{fandango!75}& \cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{White!50} &\cellcolor{teal} &\cellcolor{fandango!75}  & \cellcolor{teal}&\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{teal} &  \cellcolor{White!50}   \\
143F &\cellcolor{teal} & \cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{teal} &\cellcolor{teal} & \cellcolor{teal}& \cellcolor{teal}& \cellcolor{teal}&\cellcolor{fandango!75} & \cellcolor{teal}&\cellcolor{teal}  &\cellcolor{fandango!75} &\cellcolor{teal} &\cellcolor{fandango!75}     \\
\midrule
\end{tabular}
\vspace{-0.2cm}
\caption{Color coding of the typological diversity of the train and test languages w.r.t. different features. Languages with the same color have the same feature value for that task (excluded languages are left blank).}
\label{table:variation}
\end{table}

